A FIRM Approach to Software-Defined Service Composition

Service composition is an aggregate of services often leveraged to automate the enterprise business processes. While Service Oriented Architecture (SOA) has been a forefront of service composition, services can be realized as efficient distributed and parallel constructs such as MapReduce, which are not typically exploited in service composition. With the advent of Software\-Defined Networking (SDN), global view and control of the entire network is made available to the networking controller, which can further be leveraged in application level. This paper presents FIRM, an approach for Software-Defined Service Composition by leveraging SDN and MapReduce. FIRM comprises Find, Invoke, Return, and Manage, as the core procedures in achieving a QoS-Aware Service Composition.

==> backup.tex <==
Below information can be retrieved:
 * Configuration data nodes"
------------------------------------------- 
 The list of configured interfaces on the device.
 
 Physical address
  "The interface's address at its protocol sub-layer. For
example, for an 802.x interface, this object normally
contains a Media Access Control (MAC) address. The
interface's media-specific modules must define the bit

speed
 units "bits/second";
description
"An estimate of the interface's current bandwidth in bits
per second. For interfaces that do not vary in
bandwidth or for those where no accurate estimation can
be made, this node should contain the nominal bandwidth.
For interfaces that have no concept of bandwidth, this
node is not present.";


 "For packet-oriented interfaces, the number of outbound
packets that could not be transmitted because of errors.
For character-oriented or fixed-length interfaces, the
number of outbound transmission units that could not be
transmitted because of errors.


 "The number of outbound packets that were chosen to be
discarded even though no errors had been detected to
prevent their being transmitted. One possible reason
for discarding such a packet could be to free up buffer
space.



https://github.com/opendaylight/yangtools/blob/master/model/ietf/ietf-interfaces/src/main/yang/ietf-interfaces.yang#L455


"Switching Capabilities of an interface.";
 "Path Computation Capabilities.";
 
  "Identifier to uniquely identify a node in TED";
  
   ted-link-attributes {

==> backup_implementation.tex <==
%				\vspace{-0.7em}

The Weather Search System is a simple MapReduce application that lets the users analyze the weather information. The system gets the weather data in the form of log files. A log file contains multiple lines depicting the weather information in the format, {city, date, hour, temperature, humidity, rainfall} as, Lisboa,2012-10-25,00:00,10,60,0 


\begin{figure}[ht]
	\begin{center}
			\resizebox{\columnwidth}{!}{
				\includegraphics[width=\textwidth]{mr.png}
			}
		\end{center}
		\caption{The deployment architecture}
		\label{fig:depl}
	\end{figure}


We have a cluster of 100 computing nodes (hosts). We also have a few map() executing independently from a few instances. Now, for the reduce() functions, the intermediate results may need to be sent to other instances.


ResourceManager and NameNode act as the two master nodes of Hadoop. ResourceManager manages the available resources in the Hadoop cluster. NameNode stores the meta data of the all the nodes. Moreover, a MapReduce Job History Server is dedicated to store and offer the historical information on MapReduce invocations. All the other nodes function as the DataNodes which also consist of the NodeManager responsible for its own resource allocation. There will be a communication across the DataNodes and NameNode throughout for management and control information. 

The file is read by the client into one of the master nodes, namingly ResourceManager. Further, the file is partitioned and stored into HDFS. The map reduce application retrieves the log files, and enters the weather information to the database. 

The Mapper class, WeatherMapper consisting of Map() takes lines from the input file and outputs $<K,V>$ pairs, of K being a Text "City,Date”, and V a custom class named WValue, containing three doubles - temperature, humidity, and rainfall.

The Reducer class WeatherReducer consisting of Reduce(), takes the output of the mapper and calculates the statistics. The output of the reducer is <"city,date" , Wstatistics>. This is final statistical information of the weather data from the data analysed for each city and date.

Here Wstatistics gives the statistical information of past weather events for any given city for the given day.
(LongWritable, Text) → [Mapper] → (Text, WValue) → [Reducer] → (Text, Text)

In this application, many map() functions will be executed at multiple Hadoop instances. Further reduce() functions will also be executed at the instances, at a latter stage. Here in fact, all the map() and reduce() can co-exist inside a single Hadoop instance hosted in a single machine. But we need scalability. Hence we deploy a cluster.

A MapReduce cluster is a Hadoop cluster formed across a local network. The network consists of multiple switches in a tree topology. Each switch is connected to a few hosts. Each host consists of an executing Hadoop instance. In this distributed deployment of Hadoop, the map() functions and reduce() functions execute independently. However, the final results are combined. 

Each node runs its own JVM. Resource Manager instance manages the resources and task allocation and distribution. Communication across the nodes are minimized by attempting to execute the Map() and reduce() inside the same node on the data partitions of the instance. However, the communication cannot be avoided altogether, as there will be communication between each node and the management node, which will be a traffic flow of many origins to a single destination (management node), and single origin (management node) to many destinations.


The network can have many origin nodes for the flows, which are sent to many different destinations. In the final stage, the flows can be sent to the single node.


\textbf{Deployment: }
A physical deployment would consist of \\
1. OpenDaylight Controller.\\
2. SDN Switches.\\
3. Hosts (computers) with Hadoop installations.\\

Due to the limited availability of having a large number of SDN switches and nodes for a real MapReduce clustered environment expeced in this application scenario, an emulation environment will be used. As a Hadoop cluster cannot be directly executed on Mininet emulated environment, we will emulate the MapReduce workflows  through Iperf based emulations.

Hence, we have the below emulated deployment.\\
1. OpenDaylight Controller.\\
2. Emulated SDN Switches and Hosts.\\
3. MapReduce execution emulated by Iperf.\\

OpenDaylight is responsible for setting the initial flowtables in each switches in a typical scenario, and is oblivious of the subsequent workflows or flows/packets. We are proposing an extension, which makes the controller aware of the service compositions. Hence, the workload routing through the nodes can be chosen to be adaptive, to minimize the work load, congestion, or to pick the shortest path.

The flows are processed by the controller, based on the information readily available to the controller, and through the information that we will periodically be sending to the controller. Congestion on the routes, health in the hosts, locality of the instance.

Hence, with the deployment of an SDN aware of the network that the MapReduce cluster is deployed on, we attempt to develop a self-adaptive MapReduce cluster that uses the knowledge of the network readily available to the controller in configuring and re-configuring the data partitions effectively. 

The SDN MapReduce deployment can be self-healing during failures or malfunctioning of a few nodes.


==> related_work_bk.tex <==
Middleware platforms empower the developers and users with an additional layer, enhancing scalability and performance. Enterprise applications are often managed and controlled by a middleware layer. 

As a MapReduce implementation, Hadoop executes Map() and Reduce() functions in multiple nodes. As the data shuffled between the invocation of Map() and Reduce(), there is always a communication across the nodes, causing delays and bandwidth overhead. The network-wide information can be retrieved through the SDN controller such as the flows transferred and hence deriving further details on congestion and load balancing across multiple different paths in the deployment. 

Moreover, Hadoop offers the Hadoop Distributed File System (HDFS) that leverages the storage space across multiple computing nodes. While providing a large storage space distributed across multiple hard drives, HDFS offers a logically unified view of a large computational disk. Hence, much larger files that cannot be stored in a single disk of a utility computer can effectively be stored across an HDFS.

In a typical word processing scenario, a client node reads the file and loads it into the HDFS. HDFS cluster is composed of multiple nodes executing Hadoop. Hadoop HDFS consists of a NameNode as well as DataNodes. DataNodes store the distributed data offering a distributed storage, where NameNode manages the metadata of the filesystem. Rack awareness feature of Hadoop offers a fault-tolerant deployment of a Hadoop cluster by copying the replicates of the data objects in a physically separated rack. Hence, fault-tolerant data centers can be built with Hadoop.


